IRS-Aided SWIPT: Joint Waveform, Active and Passive Beamforming Design Under Nonlinear Harvester Model

The performance of Simultaneous Wireless Information and Power Transfer (SWIPT) is mainly constrained by the received Radio-Frequency (RF) signal strength. To tackle this problem, we introduce an Intelligent Reflecting Surface (IRS) to compensate the propagation loss and boost the transmission efficiency. This paper proposes a novel IRS-aided SWIPT system where a multi-carrier multi-antenna Access Point (AP) transmits information and power simultaneously, with the assist of an IRS, to a single-antenna User Equipment (UE) employing practical receiving schemes. Considering harvester nonlinearity, we characterize the achievable Rate-Energy (R-E) region through a joint optimization of waveform, active and passive beamforming based on the Channel State Information at the Transmitter (CSIT). This problem is solved by the Block Coordinate Descent (BCD) method, where we obtain the active precoder in closed form, the passive beamforming by the Successive Convex Approximation (SCA) approach, and the waveform amplitude by the Geometric Programming (GP) technique. To facilitate practical implementation, we also propose a low-complexity design based on closed-form adaptive waveform schemes. Simulation results demonstrate the proposed algorithms bring considerable R-E gains with robustness to CSIT inaccuracy and finite IRS states, and emphasize the importance of modeling harvester nonlinearity in the IRS-aided SWIPT design.

==> assets/antenna_equivalent_circuit.tex <==
\begin{circuitikz}[transform shape]
	\draw (0,0) to [sV=$v_{\mathrm{S}}$] (0,2);
	\draw (0,2) to [short] (1,2);
	\draw (1,2) to [R=$R_{\mathrm{A}}$] (3,2);
	\draw (3,2) to [short] (4,2);
	\draw (4,2) to [R=$R_{\mathrm{in}}$, v<=$v_{\mathrm{in}}$] (4,0);
	\draw (4,0) to [short] (2,0) node[ground](GND){};
	\draw (2,0) to [short] (0,0);
\end{circuitikz}


==> assets/ps_receiver.tex <==
\begin{circuitikz}[transform shape]
	\draw (0,0) node[bareRXantenna](r){Rx}(r.center)
		to[short,-o] ++(0,-1)
		to node[coupler,anchor=left up](c){Power Splitter} ++(1,0);
	\draw (c.right up)
		to[short,-o] ++(0.5,0) node[above right]{$1-\rho$}
		to ++(0,0.5)
		to ++(1,0)
		to node[draw,minimum height=2em,minimum width=10em,anchor=west]{Information Decoder} ++(0,0);
	\draw (c.right down)
		to[short,-o] ++(0.5,0) node[below right]{$\rho$}
		to ++(0,-0.5)
		to ++(1,0)
		to node[draw,minimum height=2em,minimum width=10em,anchor=west]{Energy Harvester} ++(0,0);
\end{circuitikz}


==> assets/ts_receiver.tex <==
\begin{circuitikz}[transform shape]
	\draw (0,0) node[bareRXantenna](r){Rx}(r.center)
		to[short,-o] ++(0,-1) node[below]{Time Switcher}
		to[short] node[spdt,anchor=in](s){} ++(0.5,0);

	\draw (s.out 1) node[above right]{$1-\eta$}
		to ++(1.25,0)
		to ++(0,0.5)
		to ++(1,0)
		to node[draw,minimum height=2em,minimum width=10em,anchor=west]{Information Decoder} ++(0,0);

	\draw (s.out 2) node[below right]{$\eta$}
		to ++(1.25,0)
		to ++(0,-0.5)
		to ++(1,0)
		to node[draw,minimum height=2em,minimum width=10em,anchor=west]{Energy Harvester} ++(0,0);
\end{circuitikz}

